Comparison Conundrum and the Chamber of Visualizations: An Exploration of How Language Influences Visual Design

The language for expressing comparisons is often complex and nuanced, making supporting natural language-based visual comparison a non-trivial task. To better understand how people reason about comparisons in natural language, we explore a design space of utterances for comparing data entities. We identified different parameters of comparison utterances that indicate what is being compared (i.e., data variables and attributes) as well as how these parameters are specified (i.e., explicitly or implicitly). We conducted a user study with sixteen data visualization experts and non-experts to investigate how they designed visualizations for comparisons in our design space. Based on the rich set of visualization techniques observed, we extracted key design features from the visualizations and synthesized them into a subset of sixteen representative visualization designs. We then conducted a follow-up study to validate user preferences for the sixteen representative visualizations corresponding to utterances in our design space. Findings from these studies suggest guidelines and future directions for designing natural language interfaces and recommendation tools to better support natural language comparisons in visual analytics.

==> README <==
Created by Torsten Moeller (vis@cs.sfu.ca), April 6 2004
modified by Steven Bergner and Torsten Moeller, June 30 2006
modified by James Peltier and Torsten Moeller, March 28, 2007
modified by Bernhard Finkbeiner, July 5, 2010
modified by Tobias Isenberg, January 2016
modified by Filip Sadlo, March 2016
modified by Tobias Isenberg, July 2016

This distribution provides a document class for formatting papers according to the specifications for submission to conferences sponsored by the IEEE Visualization & Graphics Technical Committee (VGTC).

Conferences that use the 'journal' document option:
- IEEE Visualization Conference (VIS, incl. InfoVis, SciVis, VAST)
- IEEE Virtual Reality (VR)
- IEEE International Symposium on Mixed and Augmented Reality (ISMAR)

It contains 13 files/directories:

README          - this file
diamondrule.eps - abstract and body separator
diamondrule.pdf - its PDF version
vgtc.cls        - the VGTC class file, which should be placed, somewhere in the TeX search path (or in the local directory)
template.tex    - an example paper
template.bib    - a small bibliography file used by the example
template.pdf    - an example proper pdf output in default journal mode
abbrv-doi*.bst  - four different versions to generate the bibliography including DOI output, with and without hyperref support, with and without narrow rendering of DOIs
makefile        - makefile including bibtex compilation and proper PDF generation
pictures/       - subdirectory with sample images, both in EPS and in direct pixel/vector format

Usage
=====

The template can be used as such (using the established LaTeX environments) by calling pdfLaTeX or LaTex. For Windows-based LaTeX installations you can use, for example, the environment provided by http://www.texniccenter.org/ along with MikTeX (http://miktex.org/). For Uinux-based installations, please use your favorite LaTeX distribution and editing environment or use the makefile following the instructions below.

Use of the Makefile
===================

Prior to "building" a paper please be sure to run

  make clean

This will ensure that the paper is built cleanly each and every time. We suggest to run this command before each new compilation.

To compile the example, run

  make

or manually, if the makefile does not work for you

  latex template
  bibtex template
  latex template
  latex template

If you run 'make' for the first time, a successful compilation will create a file called 'template.pdf'. Please make sure, that its layout is identical to the file 'template-journal.pdf' provided with this package.

The included makefile also allows you to run each step of the process manually.  Below are a list of available options that may be passed to make

 "make clean"
   removes all files that can be generated automatically.

 "make gs7"
   This will perform all functions to build a proper paper using GhostScript 7.

 "make gs8"
   This will perform all functions to build a proper paper using GhostScript 8.

 "make dvi"
   This will process the .tex file and produce a DVI output file.  This
   step may process the .tex file several times to process all references
   and citations.

 "make ps"
   This will process the .tex file and the DVI output and convert it to a
   PostScript file.

 "make pdf"
   This will process the .tex file using pdfTeX/pdflatex to produce a PDF
   file directly (not using a DVI and PostScript file).
   Please make sure that all fonts are embedded.
   You can use pdffonts my_document.pdf to check if they are.
   It is standard in all modern latex distributions.
   If you use eps figures (e.g. R or gnuplot figures) which you convert to
   PDF using epstopdf, do the following:
   Use GL_OPTIONS, a global environment variable for ghostscript:
   export GS_OPTIONS="-dEmbedAllFonts=true -dPDFSETTINGS=/printer"
   # and run
   epstopdf myfile.eps

   See http://bugs.debian.org/cgi-bin/bugreport.cgi?bug=411651 for the
   origin of this solution.


If you have problems with the makefile please notify us with the output of
the errors produced when running make and we will work to figure out the
resolution.


To produce proper pdf output, please use:
  dvips -t letter -Pdownload35 -Ppdf -G0 template.dvi -o template.ps

The "-Ppdf" and "-G0" flags should be specified in that order; reversing
them does not work, and will result in unacceptable results.

The following information is an exerpt from the ACM SIGGRAPH Conference /
Symposium / Workshop Content Formatting Instructions which can be found
here.

 http://www.siggraph.org/publications/instructions/author-instructions.pdf

If you are using version 7.x of GhostScript, please use the following
method of invoking ‘ps2pdf,’ in order to embed all typefaces and ensure
that images are not downsampled or subsampled in the PDF creation process:

 ps2pdf -dCompatibilityLevel=1.3 -dMaxSubsetPct=100 \
        -dSubsetFonts=true -dEmbedAllFonts=true \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

If you are using version 8.x of GhostScript, please use this method in
place of the example above:

 ps2pdf -dPDFSETTINGS=/prepress -dCompatibilityLevel=1.3 \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

This has been incorporated into the makefile and should no longer be needed
unless you are building the PDF file manually.


==> makefile <==
# This file seems to originate from something called 'the ultimate
# latex makefile' that different authors worked on. Find original
# versions at:
# http://tadek.pietraszek.org/blog/2006/03/24/the-ultimate-latex-makefile/
# (c) by Tadeusz Pietraszek
# http://www.acoustics.hut.fi/u/mairas/UltimateLatexMakefile/ 
# (c) by Matti Airas
#
# This file has been assembled and adjusted by Steven Bergner, Nov 2005
#  - support for multiple sub-texfiles
#  - fixed '=' '#' problem in mingw/msys environment (see E variable)
#  - PS compilation uses VGTC recommended settings
#  - targets restructured to make PDF by default
#
# Call 'make dvi' for minimal compilation, to check for proper latex
# syntax. This can be much faster than a full PDF generation when big
# figures are involved.
#
# Call 'make pdf' for direct compilation to PDF using pdfTeX. Note that this
# requires you to use .pdf files. pdfTeX can not use .ps or .eps graphics.
# use epstopdf to convert such files to .pdf files.
#
#----------------------------------------------------------------------------
#adjust the following for your purpose

#set the a .dvi name that corresponds to your main .tex file
DVIFILES = template.dvi
MAINTEXFILE = $(DVIFILES:.dvi=.tex)
SUBTEXFILES = 
BIBFILES = template.bib

#switch = to # when using ps2pdf in win32 (mingw/msys), i.e. uncomment 2nd line
#E=\=
E=\#

#adjust paper size: letter/a4
PAPERSIZE=letter
PDFLATEXPAPERSIZE="-sPAPERSIZE$E$(PAPERSIZE)"
DVIPSPAPERSIZE=-t $(PAPERSIZE)
#uncomment the following two lines when using option tvcgpapersize
#DVIPSPAPERSIZE=-T 7.875in,10.75in
#PDFLATEXPAPERSIZE=

#----------------------------------------------------------------------------
LATEX = latex
BIBTEX = bibtex
L2H = latex2html
PDFLATEX = ps2pdf
PDFTEX = pdflatex
DVIPS = dvips 

RERUN = "(There were undefined references|Rerun to get (cross-references|the bars) right)"
RERUNBIB = "No file.*\.bbl|Citation.*undefined" 

PSFILES  = $(DVIFILES:.dvi=.ps) 

PDFFILES7 = $(DVIFILES:.dvi=.pdf7) 
PDFFILES8 = $(DVIFILES:.dvi=.pdf8) 

PDFTEXFILES = $(DVIFILES:.dvi=.pdftex)

COPY = if test -r $*.toc; then cp $*.toc $*.toc.bak; fi 
#RM = /usr/bin/rm -f 
RM = rm -f 

all:	msg gs8

msg:
	@echo "  This script defaults to GhostScript 8.  If you are using GhostScipt 7 please type"
	@echo "  make gs7 instead.  If unsure type gs -v from the command line"
	@echo "  To use pdflatex/pdftex, type make pdf"
	@echo ""


pdf:     clean pdftex 

gs7:        clean dvi ps pdf7

gs8:        clean dvi ps pdf8

dvi:           $(DVIFILES)

ps:           $(PSFILES)

pdf7:           $(PDFFILES7)

pdf8:           $(PDFFILES8)

pdftex:         $(PDFTEXFILES)

$(MAINTEXFILE) : $(SUBTEXFILES) $(BIBFILES)

%.dvi:			%.tex
				$(COPY);$(LATEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(LATEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.pdftex:			%.tex
				echo "wir sind da"
				$(COPY);$(PDFTEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(PDFTEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.ps:			%.dvi
#				dvips -T 7.875in,10.75in -Ppdf -G0 $< -o $@  #use tvcgpapersize
#				dvips -Ppdf -G0 $< -o $@
				dvips $(DVIPSPAPERSIZE) -Pdownload35 -Ppdf -G0 $< -o $@
#				dvips $< -o $@


%.pdf7:			%.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dMaxSubsetPct$E100" \
	"-dCompatibilityLevel$E1.3" \
	"-dSubsetFonts$Etrue" \
	"-dEmbedAllFonts$Etrue" \
	"-dAutoFilterColorImages$Efalse" \
	"-dAutoFilterGrayImages$Efalse" \
	"-dColorImageFilter$E/FlateEncode" \
	"-dGrayImageFilter$E/FlateEncode" \
	"-dMonoImageFilter$E/FlateEncode" \
	$< template.pdf

#				$(PDFLATEX) $<

%.pdf8:                 %.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dPDFSETTINGS=/prepress" \
	"-dCompatibilityLevel=1.3" \
	"-dAutoFilterColorImages=false" \
	"-dAutoFilterGrayImages=false" \
	"-dColorImageFilter=/FlateEncode" \
	"-dGrayImageFilter=/FlateEncode" \
	"-dMonoImageFilter=/FlateEncode" \
	"-dDownsampleGrayImages=false" \
	"-dDownsampleColorImages=false" \
	$< template.pdf
#                               $(PDFLATEX) $<

# cleans anything that can be re-generated automatically, plus emacs backups
clean: 
				rm -f *.aux *.log *.bbl *.blg *.brf *.cb *.ind *.idx *.ilg	\
				*.inx *.toc *.out $(DVIFILES) $(PSFILES) template.pdf *~

.PHONY : all pdf ps dvi clean $(MAINTEXFILE)


==> sections/Exp1_DataCoding_Writing_Example.tex <==

In total, we collected 11 pieces of information about each paper and the empirical user experiments they contained. The categories of information which were informed by the authors' experience conducting visualization research and consulting past surveys which evaluated different types of visualizations (e.g., \cite{mack2019accessibility, hullman2018pursuit}). 
We selected these categories to capture overall characteristics of the paper (e.g., what the main contribution of the paper was) as well as details of the methodology in order to better understand what kinds of methods were being employed.

While a document containing all of the data we collected can be found in the Supplemental Materials, we summarize the information categories explicitly extracted from each paper in Table \ref{table:data}.

\begin{table}[h!btp]
\centering
\small
\setlength\tabcolsep{5pt}
\ra{1}
\maxsizebox*{\linewidth}{0.95\textheight}{%
\begin{tabularx}{\linewidth}{p{3cm} p{5cm}}
	\toprule
	\textbf{Category} & \textbf{Examples/Explanation}\\ \hline
    	\textbf{Main contribution} & Artifact, Empirical, Methodology, Theoretical (based on \cite{wobbrock201contributions})\\ \arrayrulecolor{lightgray} \hline
		\textbf{Type of experiment} & Experiment only, Iterative design, \newline Participatory design, Need-finding \\ \hline
		\textbf{Intended audience} & Novices, General public, Decision Makers \\ \hline
		\textbf{Num. of participants} & A number or unclear  \\ \hline
		\textbf{Type of participants} & Students, Community members, \newline Crowdworkers \\ \hline
		\textbf{Data dimensions} &  \# of dimensions  (based on \cite{iliinsky2011complexity}) \\ \hline
		\textbf{Data authenticity} & Real, Synthetic, Unknown \\ \hline
		\textbf{Type of visualization} & Bar chart, Line chart, Scatterplot  \\ \hline
		\textbf{Visualization \newline interactivity} & Interactive, Static, Animated  \\ \hline
		\textbf{Evaluation measures} & \# of correct answers, Time, Perceived ease of use  \\ \hline
		\textbf{Elicitation methods} & Self-reported, Observation, Trace Records  \\
		
	\arrayrulecolor{black}\bottomrule
\end{tabularx}}
\caption{We collected 11 pieces of information about the content of each paper ranging from the main contribution of the paper to the specific methods used to elicit information from participants.}
\label{table:data}
\vspace{-5mm}
\end{table}

==> sections/conclusion.tex <==
\section{Conclusion}
Visual comparisons are an important form of analytical workflows as people reason about and make sense of data. With the growing popularity of NLIs and recommendation systems, interpreting and visualizing the semantic nuances of comparison utterances can be challenging. In this paper, we explore a preliminary design space of NL comparison utterances covering four cardinalities of comparisons and addressing varying degrees of concreteness in these comparison intents. Through a series of interviews with 16 visualization novices and experts, we create a potential mapping between comparison utterances in our design space and different visualization techniques. By empirically validating this mapping in a preference ranking study with 77 participants, we provide design \hl{implications} for interpreting comparison language for a range of scenarios. We hope that our findings are a step towards addressing the complex interplay between language and visualization.


==> tables/study-1-conditions.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}

% \begin{table*}
% \centering
% % \resizebox{\textwidth}{!}{
% \begin{tabular}{|lc|ll|ll|p{10.3cm}|}
% \hline
% \multicolumn{2}{|c|}{
% } & \multicolumn{2}{c|}{
% Data Value(s)} & \multicolumn{2}{c|}{
% Data Attribute(s)} & \multicolumn{1}{c|}{
% } \\
 
% \multicolumn{2}{|c|}{\multirow{-2}{*}{
% Qid}} & &

% & &
% & \multicolumn{1}{c|}{\multirow{-2}{*}{
% Example Query}} \\ \hline\hline
% \multicolumn{1}{|l|}{A} &  & \multicolumn{2}{c|}{explicit} & \multicolumn{2}{c|}{explicit} & compare the imdb ratings of squid game and midnight mass \\ \cline{1-1} \cline{3-7} 
% \multicolumn{1}{|l|}{B} &  & \multicolumn{2}{c|}{explicit} & \multicolumn{2}{c|}{implicit} & compare the performance of squid game and midnight mass \\ \cline{1-1} \cline{3-7} 
% \multicolumn{1}{|l|}{C} &  & \multicolumn{2}{c|}{implicit} & \multicolumn{2}{c|}{explicit} & compare the box office numbers of a high rated movie made in US to a high rated movie made in India \\ \cline{1-1} \cline{3-7} 
% \multicolumn{1}{|l|}{D} & \multirow{-4}{*}{1-1} & \multicolumn{2}{c|}{implicit} & \multicolumn{2}{c|}{implicit} & compare the popularity of a high budget movie to a low budget movie \\ \hline
% \multicolumn{1}{|l|}{A} &  & \multicolumn{2}{c|}{explicit} & \multicolumn{2}{c|}{explicit} & compare the amount of times squid game was watched as opposed to all other thriller tv shows \\ \cline{1-1} \cline{3-7} 
% \multicolumn{1}{|l|}{B} &  & \multicolumn{2}{c|}{explicit} & \multicolumn{2}{c|}{implicit} & compare the performance of Starling to other PG-13 movies \\ \cline{1-1} \cline{3-7} 
% \multicolumn{1}{|l|}{C} &  & \multicolumn{2}{c|}{implicit} & \multicolumn{2}{c|}{explicit} & compare a high rated movie with similar high rated movies in terms of box office \\ \cline{1-1} \cline{3-7} 
% \multicolumn{1}{|l|}{D} & \multirow{-4}{*}{1-n} & \multicolumn{2}{c|}{implicit} & \multicolumn{2}{c|}{implicit} & compare a low budget tv show to other low budget tv shows with respect to their popularity \\ \hline
% \multicolumn{1}{|l|}{A} &  & \multicolumn{2}{c|}{explicit} & \multicolumn{2}{c|}{explicit} & compare the budgets across all US movies \\ \cline{1-1} \cline{3-7} 
% \multicolumn{1}{|l|}{B} &  & \multicolumn{2}{c|}{explicit} & \multicolumn{2}{c|}{implicit} & compare the performances across all US movies \\ \cline{1-1} \cline{3-7} 
% \multicolumn{1}{|l|}{C} &  & \multicolumn{2}{c|}{implicit} & \multicolumn{2}{c|}{explicit} & compare the box office numbers for all high rated movies \\ \cline{1-1} \cline{3-7} 
% \multicolumn{1}{|l|}{D} & \multirow{-4}{*}{n} & \multicolumn{2}{c|}{implicit} & \multicolumn{2}{c|}{implicit} & compare the performances of all shows with long runtime \\ \hline
% \multicolumn{1}{|l|}{A} &  & \multicolumn{2}{c|}{explicit} & \multicolumn{2}{c|}{explicit} & compare crime tv shows to thriller tv shows in terms of budget \\ \cline{1-1} \cline{3-7} 
% \multicolumn{1}{|l|}{B} &  & \multicolumn{2}{c|}{explicit} & \multicolumn{2}{c|}{implicit} & compare the popularity of Documentaries to Comedies \\ \cline{1-1} \cline{3-7} 
% \multicolumn{1}{|l|}{C} &  & \multicolumn{2}{c|}{implicit} & \multicolumn{2}{c|}{explicit} & compare the box office numbers between high rated movies and high rated tv shows \\ \cline{1-1} \cline{3-7} 
% \multicolumn{1}{|l|}{D} & \multirow{-4}{*}{n-n} & \multicolumn{2}{c|}{implicit} & \multicolumn{2}{c|}{implicit} & compare the performance of movies with long runtime in the US and Europe \\ \hline
% \end{tabular}
% \label{table:code_netflix}
% \end{table*}

==> tables/study2-results.tex <==
% \makeatletter
% \newsavebox\saved@arstrutbox
% \newcommand*{\setarstrut}[1]{%
%   \noalign{%
%     \begingroup
%       \global\setbox\saved@arstrutbox\copy\@arstrutbox
%       #1%
%       \global\setbox\@arstrutbox\hbox{%
%         \vrule \@height\arraystretch\ht\strutbox
%               \@depth\arraystretch \dp\strutbox
%               \@width\z@
%       }%
%     \endgroup
%   }%
% }
% \newcommand*{\restorearstrut}{%
%   \noalign{%
%     \global\setbox\@arstrutbox\copy\saved@arstrutbox
%   }%
% }
% \makeatother

% \newcolumntype{C}[1]{>{\centering\arraybackslash}m{#1}}
% \begin{table}[h!]
%     % \begin{tabular}{|m{2cm}|m{7cm}|m{3cm}|}
%     \setlength\extrarowheight{2pt}
%     \centering
%     \begin{tabular}{|C{0.83cm}|C{0.83cm}|C{0.83cm}|C{0.83cm}|C{0.83cm}|C{0.83cm}|C{0.83cm}|}
%     \hline
%         \cellcolor{gray!30}\OnetoOne & \cellcolor{gray!30}A, B & \cellcolor{gray!30}A, C & \cellcolor{gray!30}A, D & \cellcolor{gray!30}B, C & \cellcolor{gray!30}B, D & \cellcolor{gray!30}C, D \\ \hline
%         \EVEA & {\small p\:$>$\:0.05} & {\small \cellcolor{blue!40} p\:$<$\:0.001} & {\small \cellcolor{blue!40} p\:$<$\:0.001} & {\small \cellcolor{blue!15} p\:$<$\:0.05} & {\small \cellcolor{blue!40} p\:$<$\:0.001} & {\small  p\:$>$\:0.05} \\ \hline
%         \EVIA & {\small  p\:$>$\:0.05} & {\small \cellcolor{blue!40} p\:$<$\:0.001} & {\small \cellcolor{blue!40} p\:$<$\:0.001} & {\small  p\:$>$\:0.05} & {\small  p\:=\:1.00} & {\small  p\:=\:1.00} \\ \hline
%         \IVEA & {\small  p\:$>$\:0.05} & {\small \cellcolor{blue!40} p\:$<$\:0.001} & {\small \cellcolor{blue!40} p\:$<$\:0.001} & {\small \cellcolor{blue!40} p\:$<$\:0.001} & {\small \cellcolor{blue!40} p\:$<$\:0.001} & {\small  p\:=\:1.00} \\ \hline
%         \IVIA & {\small  p\:$>$\:0.05} & {\small \cellcolor{blue!25} p\:$<$\:0.01} & {\small \cellcolor{blue!25} p\:$<$\:0.01} & {\small  p\:$>$\:0.05} &  {\small  p\:$>$\:0.05} &  {\small  p\:=\:1.00} \\ \hline
        
%         \setarstrut{\tiny}%
%         \multicolumn{7}{c}{{\tiny\textbf{}}} \\\hline
%         \restorearstrut
        
%         \cellcolor{gray!30}\OnetoN & \cellcolor{gray!30}E, F & \cellcolor{gray!30}E, G & \cellcolor{gray!30}E, H & \cellcolor{gray!30}F, G & \cellcolor{gray!30}F, H & \cellcolor{gray!30}G, H \\ \hline
%         \EVEA & {\small \cellcolor{blue!15} p\:$<$\:0.05} & {\small \cellcolor{blue!40} p\:$<$\:0.001} & {\small \cellcolor{blue!40} p\:$<$\:0.001} & {\small  p\:$<$\:0.05} & {\small  \cellcolor{blue!40}p\:$<$\:0.001} & {\small  p\:$>$\:0.05} \\ \hline
%         \EVIA & {\small \cellcolor{blue!15} p\:$<$\:0.05} & {\small \cellcolor{blue!40} p\:$<$\:0.001} & {\small \cellcolor{blue!40} p\:$<$\:0.001} & {\small  p\:$<$\:0.05} & {\small  \cellcolor{blue!40}p\:$<$\:0.001} & {\small  p\:$>$\:0.05}  \\ \hline
%         \IVEA & {\small  p\:$>$\:0.05} & {\small \cellcolor{blue!40} p\:$<$\:0.001} & {\small \cellcolor{blue!40} p\:$<$\:0.001} & {\small \cellcolor{blue!40} p\:$<$\:0.001} & {\small \cellcolor{blue!40} p\:$<$\:0.001} &  {\small  p\:=\:1.00}\\ \hline
%         \IVIA & {\small \cellcolor{blue!25} p\:$<$\:0.01} & {\small \cellcolor{blue!40} p\:$<$\:0.001} & {\small \cellcolor{blue!40} p\:$<$\:0.001} & {\small \cellcolor{blue!40} p\:$<$\:0.001} & {\small \cellcolor{blue!40} p\:$<$\:0.001} &  {\small  p\:=\:1.00} \\ \hline
        
%         \setarstrut{\tiny}%
%         \multicolumn{7}{c}{{\tiny\textbf{}}} \\\hline
%         \restorearstrut
        
%         \cellcolor{gray!30}\N & \cellcolor{gray!30}I, J & \cellcolor{gray!30}I, K & \cellcolor{gray!30}I, L & \cellcolor{gray!30}J, K & \cellcolor{gray!30}J, L & \cellcolor{gray!30}K, L \\ \hline
%         \EVEA & {\small \cellcolor{blue!40} p\:$<$\:0.001} & {\small \cellcolor{blue!40} p\:$<$\:0.001} & {\small \cellcolor{blue!40} p\:$<$\:0.001} & {\small  \cellcolor{blue!25}p\:$<$\:0.01} & {\small \cellcolor{blue!40} p\:$<$\:0.001} & {\small  p\:$>$\:0.05} \\ \hline
%         \EVIA & {\small  p\:$>$\:0.05} & {\small \cellcolor{blue!40} p\:$<$\:0.001} & {\small \cellcolor{blue!40} p\:$<$\:0.001} & {\small \cellcolor{blue!40} p\:$<$\:0.001} & {\small \cellcolor{blue!40} p\:$<$\:0.001} & {\small  p\:$>$\:0.05}  \\ \hline
%         \IVEA & {\small \cellcolor{blue!15} p\:$<$\:0.05} & {\small \cellcolor{blue!40} p\:$<$\:0.001} & {\small \cellcolor{blue!40} p\:$<$\:0.001} & {\small \cellcolor{blue!15} p\:$<$\:0.05} & {\small \cellcolor{blue!40} p\:$<$\:0.001} & {\small \cellcolor{blue!40} p\:$<$\:0.001}  \\ \hline
%         \IVIA & {\small  p\:$>$\:0.05} & {\small \cellcolor{blue!40} p\:$<$\:0.001} & {\small \cellcolor{blue!40} p\:$<$\:0.001} & {\small \cellcolor{blue!15} p\:$<$\:0.05} & {\small \cellcolor{blue!40} p\:$<$\:0.001} & {\small \cellcolor{blue!40} p\:$<$\:0.001} \\ \hline
       
%         \setarstrut{\tiny}%
%         \multicolumn{7}{c}{{\tiny\textbf{}}} \\\hline
%         \restorearstrut
       
%         \cellcolor{gray!30}\NtoN & \cellcolor{gray!30}M, N & \cellcolor{gray!30}M, O & \cellcolor{gray!30}M, P & \cellcolor{gray!30}N, O & \cellcolor{gray!30}N, P & \cellcolor{gray!30}O, P \\ \hline
%         \EVEA & {\small  p\:=\:1.00} & {\small  p\:=\:1.00} & {\small \cellcolor{blue!40} p\:$<$\:0.001} & {\small  p\:=\:1.00} & {\small \cellcolor{blue!40} p\:$<$\:0.001} & {\small \cellcolor{blue!40} p\:$<$\:0.001} \\ \hline
%         \EVIA & {\small  p\:=\:1.00} & {\small  p\:=\:1.00} & {\small \cellcolor{blue!40} p\:$<$\:0.001} & {\small  p\:=\:1.00} & {\small \cellcolor{blue!40} p\:$<$\:0.001} & {\small \cellcolor{blue!40} p\:$<$\:0.001}  \\ \hline
%         \IVEA & {\small  p\:=\:1.00} & {\small  p\:=\:1.00} & {\small \cellcolor{blue!40} p\:$<$\:0.001} & {\small  p\:=\:1.00} & {\small \cellcolor{blue!40} p\:$<$\:0.001} & {\small \cellcolor{blue!40} p\:$<$\:0.001}  \\ \hline
%         \IVIA & {\small  p\:=\:1.00} & {\small  p\:=\:1.00} & {\small \cellcolor{blue!40} p\:$<$\:0.001} & {\small  p\:=\:1.00} & {\small \cellcolor{blue!40} p\:$<$\:0.001} & {\small  \cellcolor{blue!40}p\:$<$\:0.001} \\ \hline
%     \end{tabular}
%     \vspace{4px}
%     \caption{The specific ranking differences for each visualization (A-P) in Figure~\ref{Exp2OverallResults} computed using Conover's test with Bonferroni's correction. The darker the hue, the more statistically significant the ranking difference is.}
%     \vspace{-12px}
%     \label{tab:study2-results}
% \end{table}









% \newcolumntype{C}[1]{>{\centering\arraybackslash}m{#1}}
% \begin{table}[h]
%     % \begin{tabular}{|m{2cm}|m{7cm}|m{3cm}|}
%     \setlength\extrarowheight{2pt}
%     \centering
%     \begin{tabular}{|C{0.83cm}|C{0.83cm}|C{0.83cm}|C{0.83cm}|C{0.83cm}|C{0.83cm}|C{0.83cm}|}
%     \hline
%         \OnetoOne & A, B & A, C & A, D & B, C & B, D & C, D \\ \hline
%         \EVEA & {\small p\:=\:0.45} & {\small  p\:$<$\:0.001} & {\small  p\:$<$\:0.001} & {\small  p\:=\:0.026} & {\small  p\:$<$\:0.001} & {\small  p\:=\:0.13} \\ \hline
%         \EVIA & {\small  p\:=\:0.076} & {\small  p\:$<$\:0.001} & {\small  p\:$<$\:0.001} & {\small  p\:=\:0.57} & {\small  p\:=\:1.00} & {\small  p\:=\:1.00} \\ \hline
%         \IVEA & {\small  p\:=\:0.49} & {\small  p\:$<$\:0.001} & {\small  p\:$<$\:0.001} & {\small  p\:$<$\:0.001} & {\small  p\:$<$\:0.001} & {\small  p\:=\:1.00} \\ \hline
%         \IVIA & {\small  p\:=\:0.77} & {\small  p\:$<$\:0.01} & {\small  p\:$<$\:0.01} & {\small  p\:=\:0.14} &  {\small  p\:=\:0.46} &  {\small  p\:=\:1.00} \\ \hline
%         \OnetoN & E, F & E, G & E, H & F, G & F, H & G, H \\ \hline
%         \EVEA & {\small  p\:=\:0.037} & {\small  p\:$<$\:0.001} & {\small  p\:$<$\:0.001} & {\small  p\:=\:0.037} & {\small  p\:$<$\:0.001} & {\small  p\:=\:0.28} \\ \hline
%         \EVIA & {\small  p\:=\:0.044} & {\small  p\:$<$\:0.001} & {\small  p\:$<$\:0.001} & {\small  p\:=\:0.025} & {\small  p\:$<$\:0.001} & {\small  p\:=\:0.74}  \\ \hline
%         \IVEA & {\small  p\:=\:0.37} & {\small  p\:$<$\:0.001} & {\small  p\:$<$\:0.001} & {\small  p\:$<$\:0.001} & {\small  p\:$<$\:0.001} &  {\small  p\:=\:1.00}\\ \hline
%         \IVIA & {\small  p\:$<$\:0.01} & {\small  p\:$<$\:0.001} & {\small  p\:$<$\:0.001} & {\small  p\:$<$\:0.001} & {\small  p\:$<$\:0.001} &  {\small  p\:=\:1.00} \\ \hline
%         \N & I, J & I, K & I, L & J, K & J, L & K, L \\ \hline
%         \EVEA & {\small  p\:$<$\:0.001} & {\small  p\:$<$\:0.001} & {\small  p\:$<$\:0.001} & {\small  \cellcolor{blue!25}p\:$<$\:0.01} & {\small  p\:$<$\:0.001} & {\small  p\:$<$\:0.087} \\ \hline
%         \EVIA & {\small  p\:=\:0.60} & {\small  p\:$<$\:0.001} & {\small  p\:$<$\:0.001} & {\small  p\:$<$\:0.001} & {\small  p\:$<$\:0.001} & {\small  p\:$<$\:0.14}  \\ \hline
%         \IVEA & {\small  p\:=\:0.025} & {\small  p\:$<$\:0.001} & {\small  p\:$<$\:0.001} & {\small  p\:=\:0.011} & {\small  p\:$<$\:0.001} & {\small  p\:$<$\:0.001}  \\ \hline
%         \IVIA & {\small  p\:=\:0.13} & {\small  p\:$<$\:0.001} & {\small  p\:$<$\:0.001} & {\small  p\:=\:0.012} & {\small  p\:$<$\:0.001} & {\small  p\:$<$\:0.001} \\ \hline
%         \NtoM & M, N & M, O & M, P & N, O & N, P & O, P \\ \hline
%         \EVEA & {\small  p\:=\:1.00} & {\small  p\:=\:1.00} & {\small  p\:$<$\:0.001} & {\small  p\:=\:1.00} & {\small  p\:$<$\:0.001} & {\small  p\:$<$\:0.001} \\ \hline
%         \EVIA & {\small  p\:=\:1.00} & {\small  p\:=\:1.00} & {\small  p\:$<$\:0.001} & {\small  p\:=\:1.00} & {\small  p\:$<$\:0.001} & {\small  p\:$<$\:0.001}  \\ \hline
%         \IVEA & {\small  p\:=\:1.00} & {\small  p\:=\:1.00} & {\small  p\:$<$\:0.001} & {\small  p\:=\:1.00} & {\small  p\:$<$\:0.001} & {\small  p\:$<$\:0.001}  \\ \hline
%         \IVIA & {\small  p\:=\:1.00} & {\small  p\:=\:1.00} & {\small  p\:$<$\:0.001} & {\small  p\:=\:1.00} & {\small  p\:$<$\:0.001} & {\small  \cellcolor{blue!40}p\:$<$\:0.001} \\ \hline
%     \end{tabular}
%     \vspace{4px}
%     \caption{The specific ranking differences for each visualization (A-P) in Figure~\ref{Exp2OverallResults} computed using Conover's test with Bonferroni's correction.}
%     \label{tab:study2-results}
% \end{table}



% Copy, in case I break it.
% \newcolumntype{C}[1]{>{\centering\arraybackslash}m{#1}}
% \begin{table}[h]
%     % \begin{tabular}{|m{2cm}|m{7cm}|m{3cm}|}
%     \setlength\extrarowheight{2pt}
%     \centering
%     \begin{tabular}{|C{0.84cm}|C{0.83cm}|C{0.83cm}|C{0.83cm}|C{0.83cm}|C{0.83cm}|C{0.83cm}|}
%     \hline
%         \OnetoOne & A, B & A, C & A, D & B, C & B, D & C, D \\ \hline
%         \EVEA & {\small  p\:=\:0.447} & {\small  p\:$<$\:0.001} & {\small  p\:$<$\:0.001} & {\small  p\:=\:0.026} & {\small  p\:$<$\:0.001} & {\small  p\:=\:0.133} \\ \hline
%         \EVIA & {\small  p\:=\:0.076} & {\small  p\:$<$\:0.001} & {\small  p\:$<$\:0.001} & {\small  p\:=\:0.57} & {\small  p\:=\:1.00} & {\small  p\:=\:1.00} \\ \hline
%         \IVEA & {\small  p\:=\:0.49} & {\small  p\:$<$\:0.001} & {\small  p\:$<$\:0.001} & {\small  p\:$<$\:0.001} & {\small  p\:$<$\:0.001} & {\small  p\:=\:1.00} \\ \hline
%         \IVIA & {\small  p\:=\:0.77} & {\small  p\:=\:0.0011} & {\small  p\:=\:0.0067} & {\small  p\:=\:0.1385} &  {\small  p\:=\:0.459} &  {\small  p\:=\:1.00} \\ \hline
%         \OnetoN & E, F & E, G & E, H & F, G & F, H & G, H \\ \hline
%         \EVEA & {\small  p\:=\:0.037} & {\small  p\:$<$\:0.001} & {\small  p\:$<$\:0.001} & {\small  p\:=\:0.037} & {\small  p\:$<$\:0.001} & {\small  p\:=\:0.282} \\ \hline
%         \EVIA & {\small  p\:=\:0.044} & {\small  p\:$<$\:0.001} & {\small  p\:$<$\:0.001} & {\small  p\:=\:0.025} & {\small  p\:$<$\:0.001} & {\small  p\:=\:0.741}  \\ \hline
%         \IVEA & {\small  p\:=\:0.37} & {\small  p\:$<$\:0.001} & {\small  p\:$<$\:0.001} & {\small  p\:$<$\:0.001} & {\small  p\:$<$\:0.001} &  {\small  p\:=\:1.00}\\ \hline
%         \IVIA & {\small  p\:=\:0.00316} & {\small  p\:$<$\:0.001} & {\small  p\:$<$\:0.001} & {\small  p\:$<$\:0.001} & {\small  p\:=\:0.00036} &  {\small  p\:=\:1.00} \\ \hline
%         \N & I, J & I, K & I, L & J, K & J, L & K, L \\ \hline
%         \EVEA & {\small  p\:=\:0.00034} & {\small  p\:$<$\:0.001} & {\small  p\:$<$\:0.001} & {\small  p\:$<$\:0.00117} & {\small  p\:$<$\:0.001} & {\small  p\:$<$\:0.08737} \\ \hline
%         \EVIA & {\small  p\:=\:0.60} & {\small  p\:$<$\:0.001} & {\small  p\:$<$\:0.001} & {\small  p\:$<$\:0.001} & {\small  p\:$<$\:0.001} & {\small  p\:$<$\:0.14}  \\ \hline
%         \IVEA & {\small  p\:=\:0.02515} & {\small  p\:$<$\:0.001} & {\small  p\:$<$\:0.001} & {\small  p\:=\:0.01093} & {\small  p\:$<$\:0.001} & {\small  p\:=\:0.00039}  \\ \hline
%         \IVIA & {\small  p\:=\:0.133} & {\small  p\:$<$\:0.001} & {\small  p\:$<$\:0.001} & {\small  p\:=\:0.012} & {\small  p\:$<$\:0.001} & {\small  p\:$<$\:0.001} \\ \hline
%         \NtoM & M, N & M, O & M, P & N, O & N, P & O, P \\ \hline
%         \EVEA & {\small  p\:=\:1.00} & {\small  p\:=\:1.00} & {\small  p\:$<$\:0.001} & {\small  p\:=\:1.00} & {\small  p\:$<$\:0.001} & {\small  p\:$<$\:0.001} \\ \hline
%         \EVIA & {\small  p\:=\:1.00} & {\small  p\:=\:1.00} & {\small  p\:$<$\:0.001} & {\small  p\:=\:1.00} & {\small  p\:$<$\:0.001} & {\small  p\:$<$\:0.001}  \\ \hline
%         \IVEA & {\small  p\:=\:1.00} & {\small  p\:=\:1.00} & {\small  p\:$<$\:0.001} & {\small  p\:=\:1.00} & {\small  p\:$<$\:0.001} & {\small  p\:$<$\:0.001}  \\ \hline
%         \IVIA & {\small  p\:=\:1.00} & {\small  p\:=\:1.00} & {\small  p\:$<$\:0.001} & {\small  p\:=\:1.00} & {\small  p\:$<$\:0.001} & {\small  p\:$<$\:0.001} \\ \hline
%     \end{tabular}
%     \vspace{4px}
%     \caption{The specific ranking differences for each visualization (A-P) in Figure~\ref{Exp2OverallResults} computed using Conover's test with Bonferroni's correction.}
%     \label{tab:study2-results}
% \end{table}
